Training-Free Uncertainty Estimation for Dense Regression: Sensitivity as a Surrogate

Uncertainty estimation is an essential step in the evaluation of the robustness for deep learning models in computer vision, especially when applied in risk-sensitive areas. However, most state-of-the-art deep learning models either fail to obtain uncertainty estimation or need significant modification (e.g., formulating a proper Bayesian treatment) to obtain it. Most previous methods are not able to take an arbitrary model off the shelf and generate uncertainty estimation without retraining or redesigning it. To address this gap, we perform a systematic exploration into training-free uncertainty estimation for dense regression, an unrecognized yet important problem, and provide a theoretical construction justifying such estimations. We propose three simple and scalable methods to analyze the variance of outputs from a trained network under tolerable perturbations: infer-transformation, infer-noise, and infer-dropout. They operate solely during the inference, without the need to re-train, re-design, or fine-tune the models, as typically required by state-of-the-art uncertainty estimation methods. Surprisingly, even without involving such perturbations in training, our methods produce comparable or even better uncertainty estimation when compared to training-required state-of-the-art methods.

==> source/impact.tex <==
\section*{Broader Impact}
\textcolor{black}{This paper focuses on a problem of increasing importance. In this work, we address the necessities and significance of training-free uncertainty estimation, and propose a set of simple but effective methods. We believe it will benefit a wide range of applications in deep learning, especially for areas with high risks, such as healthcare and automatic driving. The successful applications of our methods will potentially increase the robustness and reliability for these applications. For most of the previous models which fail to take the uncertainty estimation in account, our methods could serve an essential step to support a post-analysis to estimate uncertainty. Meanwhile, our work is capable of attenuating the over-confidence and reducing the bias in the models. }

==> source/reference.tex <==
\section*{References}

\small


@inproceedings{poggi2020uncertainty,
  title={On the uncertainty of self-supervised monocular depth estimation},
  author={Poggi, Matteo and Aleotti, Filippo and Tosi, Fabio and Mattoccia, Stefano},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3227--3237},
  year={2020}
}

@article{tsymbal,
  title={Deeper connections between neural networks and Gaussian processes speed-up active learning},
  author={Tsymbalov, Evgenii and Makarychev, Sergei and Shapeev, Alexander and Panov, Maxim},
  journal={arXiv preprint arXiv:1902.10350},
  year={2019}
}

@article{kendall2015bayesian,
  title={Bayesian segnet: Model uncertainty in deep convolutional encoder-decoder architectures for scene understanding},
  author={Kendall, Alex and Badrinarayanan, Vijay and Cipolla, Roberto},
  journal={arXiv preprint arXiv:1511.02680},
  year={2015}
}
@article{yang2019inferring,
  title={Inferring Distributions Over Depth from a Single Image},
  author={Yang, Gengshan and Hu, Peiyun and Ramanan, Deva},
  journal={arXiv preprint arXiv:1912.06268},
  year={2019}
}
@inproceedings{huang2018efficient,
  title={Efficient uncertainty estimation for semantic segmentation in videos},
  author={Huang, Po-Yu and Hsu, Wan-Ting and Chiu, Chun-Yueh and Wu, Ting-Fan and Sun, Min},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={520--535},
  year={2018}
}
@article{huang2017snapshot,
  title={Snapshot ensembles: Train 1, get m for free},
  author={Huang, Gao and Li, Yixuan and Pleiss, Geoff and Liu, Zhuang and Hopcroft, John E and Weinberger, Kilian Q},
  journal={arXiv preprint arXiv:1704.00109},
  year={2017}
}
@inproceedings{welling2011bayesian,
  title={Bayesian learning via stochastic gradient Langevin dynamics},
  author={Welling, Max and Teh, Yee W},
  booktitle={Proceedings of the 28th international conference on machine learning (ICML-11)},
  pages={681--688},
  year={2011}
}
@inproceedings{nix1994estimating,
  title={Estimating the mean and variance of the target probability distribution},
  author={Nix, David A and Weigend, Andreas S},
  booktitle={Proceedings of 1994 ieee international conference on neural networks (ICNN'94)},
  volume={1},
  pages={55--60},
  year={1994},
  organization={IEEE}
}

@inproceedings{AUSE,
  author    = {Eddy Ilg and
               {\"{O}}zg{\"{u}}n {\c{C}}i{\c{c}}ek and
               Silvio Galesso and
               Aaron Klein and
               Osama Makansi and
               Frank Hutter and
               Thomas Brox},
  title     = {Uncertainty Estimates and Multi-hypotheses Networks for Optical Flow},
  booktitle = {ECCV},
  pages     = {677--693},
  year      = {2018}
}

@inproceedings{TS,
  title={On calibration of modern neural networks},
  author={Guo, Chuan and Pleiss, Geoff and Sun, Yu and Weinberger, Kilian Q},
  booktitle={ICML},
  pages={1321--1330},
  year={2017}
}

@inproceedings{cohen2016group,
  title={Group equivariant convolutional networks},
  author={Cohen, Taco and Welling, Max},
  booktitle={ICML},
  pages={2990--2999},
  year={2016}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={CVPR},
  pages={248--255},
  year={2009}
}

@inproceedings{gal2017deep,
  title={Deep bayesian active learning with image data},
  author={Gal, Yarin and Islam, Riashat and Ghahramani, Zoubin},
  booktitle={ICML},
  pages={1183--1192},
  year={2017}
}

@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={MICCAI},
  pages={234--241},
  year={2015}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={CVPR},
  pages={770--778},
  year={2016}
}

@article{zwald2012berhu,
  title={The berhu penalty and the grouped effect},
  author={Zwald, Laurent and Lambert-Lacroix, Sophie},
  journal={arXiv preprint arXiv:1207.6868},
  year={2012}
}

@inproceedings{laina2016deeper,
  title={Deeper depth prediction with fully convolutional residual networks},
  author={Laina, Iro and Rupprecht, Christian and Belagiannis, Vasileios and Tombari, Federico and Navab, Nassir},
  booktitle={3DV},
  pages={239--248},
  year={2016}
}

@inproceedings{kendall2017uncertainties,
  title={What uncertainties do we need in bayesian deep learning for computer vision?},
  author={Kendall, Alex and Gal, Yarin},
  booktitle={NIPS},
  pages={5574--5584},
  year={2017}
}

@article{postels2019sampling,
  title={Sampling-free Epistemic Uncertainty Estimation Using Approximated Variance Propagation},
  author={Postels, Janis and Ferroni, Francesco and Coskun, Huseyin and Navab, Nassir and Tombari, Federico},
  journal={arXiv preprint arXiv:1908.00598},
  year={2019}
}

@article{tensorlayer2017,
author = {Dong, Hao and Supratak, Akara and Mai, Luo and Liu, Fangde and Oehmichen, Axel and Yu, Simiao and Guo, Yike},
journal = {ACM Multimedia},
title = {{TensorLayer: A Versatile Library for Efficient Deep Learning Development}},
url = {http://tensorlayer.org},
year = {2017}
}

@article{mirza2014conditional,
  title={Conditional generative adversarial nets},
  author={Mirza, Mehdi and Osindero, Simon},
  journal={arXiv preprint arXiv:1411.1784},
  year={2014}
}

@inproceedings{ledig2017photo,
  title={Photo-realistic single image super-resolution using a generative adversarial network},
  author={Ledig, Christian and Theis, Lucas and Husz{\'a}r, Ferenc and Caballero, Jose and Cunningham, Andrew and Acosta, Alejandro and Aitken, Andrew and Tejani, Alykhan and Totz, Johannes and Wang, Zehan and others},
  booktitle={CVPR},
  pages={4681--4690},
  year={2017}
}

@article{aganj2018unsupervised,
  title={Unsupervised medical image segmentation based on the local center of mass},
  author={Aganj, Iman and Harisinghani, Mukesh G and Weissleder, Ralph and Fischl, Bruce},
  journal={Scientific reports},
  volume={8},
  number={1},
  pages={13012},
  year={2018},
  publisher={Nature Publishing Group}
}

@inproceedings{he2014reshaping,
  title={Reshaping deep neural network for fast decoding by node-pruning},
  author={He, Tianxing and Fan, Yuchen and Qian, Yanmin and Tan, Tian and Yu, Kai},
  booktitle={ICASSP},
  pages={245--249},
  year={2014}
}


@article{ioffe2015batch,
  title={Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  journal={arXiv preprint arXiv:1502.03167},
  year={2015}
}

@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting},
  author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={JMLR},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014},
  publisher={JMLR. org}
}

@article{teye2018bayesian,
  title={Bayesian uncertainty estimation for batch normalized deep networks},
  author={Teye, Mattias and Azizpour, Hossein and Smith, Kevin},
  journal={arXiv preprint arXiv:1802.06455},
  year={2018}
}

@inproceedings{gal2016dropout,
  title={Dropout as a bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  booktitle={ICML},
  pages={1050--1059},
  year={2016}
}

@article{madry2017towards,
  title={Towards deep learning models resistant to adversarial attacks},
  author={Madry, Aleksander and Makelov, Aleksandar and Schmidt, Ludwig and Tsipras, Dimitris and Vladu, Adrian},
  journal={arXiv preprint arXiv:1706.06083},
  year={2017}
}

@inproceedings{chen2015deepdriving,
  title={Deepdriving: Learning affordance for direct perception in autonomous driving},
  author={Chen, Chenyi and Seff, Ari and Kornhauser, Alain and Xiao, Jianxiong},
  booktitle={ICCV},
  pages={2722--2730},
  year={2015}
}

@inproceedings{zhang2019reducing,
  title={Reducing Uncertainty in Undersampled MRI Reconstruction with Active Acquisition},
  author={Zhang, Zizhao and Romero, Adriana and Muckley, Matthew J and Vincent, Pascal and Yang, Lin and Drozdzal, Michal},
  booktitle={CVPR},
  pages={2049--2058},
  year={2019}
}

@article{silver2016mastering,
  title={Mastering the game of Go with deep neural networks and tree search},
  author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
  journal={nature},
  volume={529},
  number={7587},
  pages={484},
  year={2016},
  publisher={Nature Publishing Group}
}

@inproceedings{he2015delving,
  title={Delving deep into rectifiers: Surpassing human-level performance on imagenet classification},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={ICCV},
  pages={1026--1034},
  year={2015}
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={NIPS},
  pages={1097--1105},
  year={2012}
}

@article{binaryNN,
  title={Loss-aware binarization of deep networks},
  author={Hou, Lu and Yao, Quanming and Kwok, James T},
  booktitle={ICLR},
  year={2016}
}

@inproceedings{deepcompression,
  title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
  author={Han, Song and Mao, Huizi and Dally, William J},
  booktitle={ICLR},
  year={2015}
}

@inproceedings{maxNPN,
  title={Feed-forward Propagation in Probabilistic Neural Networks with Categorical and Max Layers},
  author={Shekhovtsov, Alexander and Flach, Boris},
  booktitle={ICLR},  
  year={2018}
}

@inproceedings{NPN,
  title={Natural-parameter networks: A class of probabilistic neural networks},
  author={Wang, Hao and Xingjian, SHI and Yeung, Dit-Yan},
  booktitle={NIPS},
  pages={118--126},
  year={2016}
}

@article{mackay1992,
  title={A practical {B}ayesian framework for backprop networks},
  author={MacKay, David},
  journal={Neural computation},
  year={1992}
}

@inproceedings{deepensemble,
  title={Simple and scalable predictive uncertainty estimation using deep ensembles},
  author={Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
  booktitle={NIPS},
  pages={6402--6413},
  year={2017}
}

@inproceedings{hinton1993,
  title={Keeping the neural networks simple by minimizing the description length of the weights},
  author={Hinton, Geoffrey E and Van Camp, Drew},
  booktitle={COLT},
  year={1993},
}
%pages={5--13},

@phdthesis{neal1995bayesian,
  title={Bayesian learning for  neural networks},
  author={Neal, Radford M},
  year={1995},
  school={University of Toronto}
}

@inproceedings{graves2011,
  author    = {Alex Graves},
  title     = {Practical Variational Inference for Neural Networks},
  booktitle = {NIPS},
  year      = {2011}
}
% pages     = {2348--2356},

@inproceedings{PBP,
  author    = {Jos{\'{e}} Miguel Hern{\'{a}}ndez{-}Lobato and
               Ryan Adams},
  title     = {Probabilistic Backpropagation for Scalable Learning of {B}ayesian Neural
               Networks},
  booktitle = {ICML},
  year      = {2015}
}
%pages     = {1861--1869},

@inproceedings{DBLP:conf/icml/BlundellCKW15,
  author    = {Charles Blundell and
               Julien Cornebise and
               Koray Kavukcuoglu and
               Daan Wierstra},
  title     = {Weight Uncertainty in Neural Network},
  booktitle = {ICML},
  year      = {2015}
}

@inproceedings{BDK,
  title={Bayesian dark knowledge},
  author={Balan, Anoop Korattikara and Rathod, Vivek and Murphy, Kevin P and Welling, Max},
  booktitle={NIPS},
  year={2015}
}



@article{DBLP:journals/corr/KingmaW13,
  author    = {Diederik P. Kingma and
               Max Welling},
  title     = {Auto-Encoding Variational {B}ayes},
  journal   = {CoRR},
  volume    = {abs/1312.6114},
  year      = {2013}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}

@misc{Authors14,
 author = {Authors},
 title = {The frobnicatable foo filter},
 note = {{BMVC14} submission ID 324. Supplied as additional material {\tt bmvc14.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {Authors},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {A. Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}
